Quantifying Divergence for Human-AI Collaboration and Cognitive Trust

Predicting the collaboration likelihood and measuring cognitive trust to AI systems is more important than ever. To do that, previous research mostly focus solely on the model features (e.g., accuracy, confidence) and ignore the human factor. To address that, we propose several decision-making similarity measures based on divergence metrics (e.g., KL, JSD) calculated over the labels acquired from humans and a wide range of models. We conduct a user study on a textual entailment task, where the users are provided with soft labels from various models and asked to pick the closest option to them. The users are then shown the similarities/differences to their most similar model and are surveyed for their likelihood of collaboration and cognitive trust to the selected system. Finally, we qualitatively and quantitatively analyze the relation between the proposed decision-making similarity measures and the survey results. We find that people tend to collaborate with their most similar models -- measured via JSD -- yet this collaboration does not necessarily imply a similar level of cognitive trust. We release all resources related to the user study (e.g., design, outputs), models, and metrics at our repo.

==> sections/future_work.tex <==
Our preliminary findings revealed variations in soft-label metrics' impact on human-machine interaction outcomes. Future work can be optimizing models within pretraining or fine-tuning to achieve improvement on specific human-model interaction outcomes. Further, models can be evaluated before real-life deployment with that perspective.
Regarding datasets that could be used in model optimization or evaluation,  we examined the commonly used method in literature, which involves aggregating diverse human annotations to capture collective human opinions (see \ref{sec:appendix}). However, aggregated group annotations do not always reflect the user's real divergence from the models. Therefore, we also raise the question regarding the reliance on aggregated human annotations as ground truth to reflect accurate human opinions on model interactions. Future research could also focus on that and data collection to accurately reflect human opinions for models at interaction.

